Gossip Dual Averaging for Decentralized Optimization of Pairwise Functions

In decentralized networks (of sensors, connected objects, etc.), there is an important need for efficient algorithms to optimize a global cost function, for instance to learn a global model from the local data collected by each computing unit. In this paper, we address the problem of decentralized minimization of pairwise functions of the data points, where these points are distributed over the nodes of a graph defining the communication topology of the network. This general problem finds applications in ranking, distance metric learning and graph inference, among others. We propose new gossip algorithms based on dual averaging which aims at solving such problems both in synchronous and asynchronous settings. The proposed framework is flexible enough to deal with constrained and regularized variants of the optimization problem. Our theoretical analysis reveals that the proposed algorithms preserve the convergence rate of centralized dual averaging up to an additive bias term. We present numerical simulations on Area Under the ROC Curve (AUC) maximization and metric learning problems which illustrate the practical interest of our approach.

==> subfiles/additional_results.tex <==
\section{Additional Results}
\label{sec:additional-results}

\subsection{Convergence of Gradient Variables}
\label{sec:conv-grad-vari}

Theorem~\ref{thm:dist_dual_averaging_general_rate} provides a convergence rate in two distinct part. First, an optimization term, which is exactly the same than in the centralized setting. Then, a network-dependent term which depends on the global variation of the dual variables; the following lemma provides an explicit dependence between this term and the topology of the network.
\begin{lemma}
  Let $W \in \bbR^{n \times n}$ be a doubly stochastic matrix satisfying~\eqref{eq:w_condition}. Let $(Z(t))_{t > 0}$ and $(G(t))_{t > 0}$ satisfying the update rule~\eqref{eq:dist_dual_matrix_update}. Then, for $t > 0$, one has:
  \[
    \left\| Z(t) - \1_n \overline{z}^n(t)^{\top} \right\| \leq \sum_{s = 1}^t \lambda_2(W)^{t - s} \|G(s - 1)\|,
  \]
  where $\lambda_2(W)$ is the second largest eigenvalue of $W$. Moreover, if $\mathcal{G}$ is connected and non bipartite and if there exists $L > 0$ such that for any $s > 0$, $\|G(s)\|_{\infty} \leq L$, then one has:
  \[
    \left\| Z(t) - \1_n \overline{z}^n(t)^{\top} \right\|_{\infty} \leq \frac{L}{1 - \lambda_2(W)}.
  \]
\end{lemma}

\subsection{Stochastic Gradient}
\label{sec:stochastic-gradient}

Again, the decentralized setting can be adapted to a stochastic setting, where each node compute an unbiased estimator of the gradient.

\begin{theorem}
  \label{thm:dist_dual_averaging_stoch_rate}
  Let $(\gamma(t))_{t \geq 0} \in (\bbR_+^*)^{\bbN}$ be a non increasing sequence. For $i \in [n]$, let $(g_i(t))_{t \geq 0} \in (\bbR^d)^{\bbN}$, $(z_i(t))_{t \geq 0} \in (\bbR^d)^{\bbN}$ and $(x_i(t))_{t > 0} \in (\bbR^d)^{\bbN}$ be generated according to Algorithm~\ref{alg:dist_dual_averaging_sto}. For $x^* \in \argmin_{x \in \mathcal{Q}} \overline{f}^n(x)$, $i \in [n]$ and $T > 0$, one has:
  \[
    \bbE_T[\overline{f}^n(\overline{x}^T_i) - \overline{f}^n(x^*)] \leq C_1(T) + C_2(T) 
  \]
  where
  \[
    \left\{
      \begin{aligned}
        C_1(T) &= \frac{1}{2 T \gamma(T)} \| x^* \|^2 + \frac{L_f^2}{2T} \sum_{t = 1}^T \gamma(t - 1) z_j(t) \| \Big] \\
        C_2(T) &=  \frac{1}{n} \sum_{j = 1}^n \bbE_t\Big[ \|z_i(t) - z_j(t) \| + \| \overline{z}^n(t) - z_j(t) \| \Big]
    \end{aligned}
    \right.
  \]
\end{theorem}

\subsection{Biased Stochastic Gradient}
\label{sec:bias-stoch-grad}

We now focus on the case where the descent direction is stochastic but also a \emph{biased} estimate of the gradient. That is, instead of updating a dual variable $z_i(t)$ with $g_i(t)$ such that $\bbE[g_i(t) | x_i(t)] \in \partial f_i(x_i(t))$, we perform some update $d_i(t)$, and we denote $\epsilon_i(t)$ the quantity such that $\bbE[d_i(t) - \epsilon_i(t) | x_i(t)] = \bbE[g_i(t) | x_i(t)] \in \partial f_i(x_i(t))$. The following theorem allows to upperbound the error induced by the bias.

\begin{theorem}
  \label{thm:dist_dual_averaging_stoch_biased_rate}
  Let $(\gamma(t))_{t \geq 0} \in (\bbR_+^*)^{\bbN}$ be a non increasing sequence. For $i \in [n]$, let $(d_i(t))_{t \geq 0} \in (\bbR^d)^{\bbN}$, $(g_i(t))_{t \geq 0} \in (\bbR^d)^{\bbN}$, $(\epsilon_i(t))_{t \geq 0} \in (\bbR^d)^{\bbN}$, $(z_i(t))_{t \geq 0} \in (\bbR^d)^{\bbN}$ and $(x_i(t))_{t > 0} \in (\bbR^d)^{\bbN}$ be generated as stated previously. For $x^* \in \argmin_{x \in \mathcal{Q}} \overline{f}^n(x)$, $i \in [n]$ and $T > 0$, one has:
  \[
    \bbE_T[\overline{f}^n(\overline{x}^T_i) - \overline{f}^n(x^*)] \leq C_1(T) + C_2(T) + C_3(T),
  \]
  where
  \[
    \left\{
      \begin{aligned}
        C_1(T) &= \frac{1}{2 T \gamma(T)} \| x^* \|^2 + \frac{L_f^2}{2T} \sum_{t = 1}^T \gamma(t - 1) \\
        C_2(T) &= \frac{L_f}{nT} \sum_{t = 1}^T \gamma(t - 1) \sum_{j = 1}^n \bbE\Big[ \|z_i(t) - z_j(t) \| + \| \overline{z}^n(t) - z_j(t) \| \Big] \\
        C_3(T) &= \frac{1}{T} \sum_{t = 1}^{T} \bbE_t[\|y(t) - x^*\| \| \overline{\epsilon}^n(t) \|].
      \end{aligned}
    \right.
  \]  
\end{theorem}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> subfiles/bias_proof.tex <==
\begin{align*}
  \bbE \Big[ \epsilon_i(t)^{\top} \theta_i(t) \Big] &=
e_i^{\top} \bbE \Bigg[\Bigg(M(t:) - \frac{\1_n \1_n^{\top}}{n} \Bigg)  G_i(\theta_i(t)) \theta_i(t) \Bigg] \\
  &= \bbE \bigg[ \bbE\Big[e_i^{\top} M(t:) G_i(\theta_i(t)) \theta_i(t) \big| {\cal F}_{t-1} \Big] \bigg]
\end{align*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../aistats_supp"
%%% End:


==> subfiles/centralized_dual_averaging.tex <==
%!TEX root = ../main_supp.tex

\section{Centralized Dual Averaging}
\label{sec:centr-dual-aver}
%\jo{the definition of $\avf$ is missing. to check in the main text}
% at this stage this is too messy to make the point clear for proximal methods... only works fine for indicators functions.

% \jo{insert prox definition here}
% Dual averaging methods was introduced in~\cite{Nesterov2009a} and extended to proximal formulations in \cite{xiao2009dual}. This algorithm is based on the following observation. In the standard proximal gradient descent (also called the forward-backward algorithm), one aims at optimizing the sum of a smooth convex function $f$ and a non-smooth regularization term $\psi$. Hence the objective is solve the problem

% \begin{equation}
% \argmin_{x \in \bbR^d} \sum_{t=1}^T f_t(x) +\psi(x) \, .
% \end{equation}
% At each step of the algorithm, one performs the following update:
% \begin{equation}
%   \label{eq:gd_update}
%   \theta(t + 1) = \prox_{\gamma(t) \psi} \Big( \theta(t) - \gamma(t) g(t)\Big),
% \end{equation}
% where $\theta(t)$ is the sequence of estimates, $\gamma(t)$ is the sequence of steps and $g(t)$ is a sequence of gradient of $ f_t$ taken at $\theta(t)$. Update~\eqref{eq:gd_update} can in fact be reformulated as follows (see for instance \cite{Parikh_Boyd13}):
% \[
%   \theta(t + 1) = \argmin_{\theta' \in \bbR^d } \left\{ f(\theta(t)) + \psi(\theta') + g(t)^{\top} \big( \theta' - \theta(t) \big) + \frac{\|\theta' -\theta(t) \|^2}{2 \gamma(t)} \right\}.
% \]
% The update step of a proximal gradient descent can thus be expressed as a minimization by leveraging a quadratic approximation of $f$ at the current estimate, with parameters $g(t)$ and $\gamma(t)$. This has connection with the work by Duchi and Singer \jo{citer Duchi and Singer 2009 }.
% % Instead of considering such a formulation

% Removing constant terms and using recursion, one has:
% \[
%   \theta(t + 1) = \argmin_{\theta' \in \mathcal{Q}} \left\{ \theta'^{\top} \sum_{s = 1}^t \gamma(s) g(s) + \frac{\|\theta' -\theta(t)\|^2}{2}  + \psi(\theta')\right\}.
% \]
% Therefore, one estimate can easily be formulated using the sequence of subgradients. However, one can notice that subgradients have decreasing weights -- since $\gamma$ is usually a decreasing sequence of non negative weights -- which is not intuitive. 



% The goal of dual averaging is to consider every subgradient with a uniform weights, by introducing the following update scheme:

\subsection{Deterministic setting}
\label{subsec:determ-sett}

The dual averaging algorithm for minimizing the sum $f+\psi$ (where $f$ is smooth, and $\psi$ is non-smooth, but its proximity operator is simple to compute) is defined in the centralized framework as follows :
\begin{align}\label{eq:def_dual_av}
\theta(t + 1) = \argmin_{\theta' \in \bbR^d } \left\{ \theta'^{\top} \sum_{s = 1}^t g(s) + \frac{\| \theta' \|^2}{2 \gamma(t)} + t \psi(\theta') \right\},
\end{align}

where $\gamma(t)$ represents a scale factor similar to a gradient step size use in standard gradient descent algorithms, and $g_t$ is a sequence of gradient of $f$ taken at $\theta(t)$. This particular formulation was introduced in \cite{xiao2009dual}, extending the method introduced by \cite{Nesterov2009a} limited to the specific case of indicator functions. We borrow the notation from \cite{xiao2009dual} in this work.

In order to perform a theoretical analysis of this algorithm, we introduce the following functions. Let us define $h$ and $V_t$ as follows:
\[
  h_t(z,\theta) = z^{\top} \theta + \frac{\| \theta \|^2}{2 \gamma(t)}  + t \psi(\theta) .
\]
% Let us define $F$ as the minimum of $g$ with respect to the first variable:
\[
V_t(z)=\displaystyle \max_{\theta \in \bbR^d} \left\{ z^{\top} \theta - \frac{\| \theta \|^2}{2 \gamma(t)}  - t \psi(\theta) \right\}
.
\]
We also define the smoothing function $\pi_t$ that plays a crucial role in the dual algorithm formulation:
\[
    \smoothop_t(z) :=  \argmax_{\theta \in \bbR^d}
    \left\{
    z^{\top} \theta - \frac{\| \theta \|^2}{2 \gamma(t)}  - t \psi(\theta) \right\}=
    \argmin_{\theta \in \bbR^d}
    \left\{
    -z^{\top}\theta + \frac{\| \theta \|^2}{2 \gamma(t)}  + t \psi(\theta) \right\}
  \]

The function $h_t(z, \cdot)$ is strongly convex in $\theta$ so the solution of the above expression is unique. The following lemma links the function $F$ and the algorithm update. The following is a simple application of the results given in \citep[Lemma 10]{xiao2009dual}:

\begin{lemma}
  \label{lma:grad_argmin}
  For any $(z, \gamma) \in \bbR^d \times \bbR_+^*$, one has:
 \begin{align}
    \smoothop_t(z) := \nabla V_t (z)
 \end{align}
   and the following holds true:
  \begin{align}
      \|    \smoothop_t(z_1)-\smoothop_t(z_2)\| \leq \gamma(t)\|z_1-z_2\| \,,
  \end{align}
and for any $g,s \in \bbR^d$,
\begin{align}\label{ineq:stongly_cvx}
V_t(z+g) \leq V_t(z) + g^\top \nabla V_t(z) + \frac{\gamma(t)}{2} \|g\|^2.
\end{align}
\end{lemma}
With this notation one can write the dual averaging rule as $\theta(t+1)=\smoothop_t \left(-s_t \right)$, where $s_t := \sum_{\tau=1}^t g_\tau$. Moreover, adapting \citep[Lemma 11]{xiao2009dual} we can state:

\begin{lemma}
For any $t\geq 1$ and any non-increasing sequence $(\gamma(t))_{t \geq 0}$, we have
\begin{align}
V_t\left(-s_t \right) + \psi(\theta_{t+1}) \leq V_t\left(-s_t \right).
\end{align}
\end{lemma}


Bounding  the regret:



\begin{theorem}
  Let $(\gamma(t))_{t \geq 0}$ be a non increasing sequence. Let $(z(t))_{t \geq 0}$, $(\theta(t))_{t > 0}$ and $(d(t))_{t > 0}$ be generated according to Algorithm~\ref{alg:dual_averaging_standard}. For $\theta^* \in \argmin_{\theta' \in \bbR^d} \avf(\theta') + \psi(\theta')$ and any $T > 0$, one has:
  \begin{equation}
    \label{eq:dual_standard_bound}
    \avf(\avtheta) + \psi (\avtheta) - \avf(\theta^*) - \psi (\theta^*)  \leq \frac{\| \theta^* \|^2}{2T \gamma(T)} + \frac{L^2}{2T} \sum_{t = 0}^{T - 1} \gamma(t).
  \end{equation}

  Moreover, if there exists $D > 0$ such that for any $y \in \mathcal{Q}$, $\|y\| \leq D$, then for $\gamma(t) = \frac{D}{L \sqrt{2t}}$, one has:
  \[
    \avf( \avtheta) - \avf(\theta^*) \leq \frac{\sqrt{2} D L}{\sqrt{T}} + \frac{L^2}{2T}.
  \]
\end{theorem}


\begin{proof}
  Let $T > 0$. Using the convexity of $\avf$, we obtain:
\begin{align*}
    \avf( \avtheta) - \avf(\theta^*) +\psi( \avtheta) - \psi(\theta^*)
    &\leq \frac{1}{T} \sum_{t = 1}^T \avf(\theta(t)) - \avf(\theta^*) +\psi( \avtheta) - \psi(\theta^*) \\
    &\leq \frac{1}{T} \sum_{t = 1}^t d(t)^{\top} (\theta(t) - \theta^*) +
    \frac{1}{T}\sum_{t = 1}^t (\psi( \avtheta(t)) - \psi(\theta^*)),
\end{align*}

Then one can check that with \eqref{ineq:stongly_cvx},
\begin{align*}
V_\tau(-\sum_{s=1}^{\tau})
\end{align*}
\end{proof}




% \begin{proof}
%   Let $(z, \gamma) \in \bbR^d \times \bbR_+^*$ and let $\theta_{z, \gamma} = \argmin_{\theta' \in \bbR^d} \left\{ z^{\top} \theta' + \frac{1}{2 \gamma} \| \theta' \|^2 +\psi(\theta')\right\}$. By definition, one has $F(z, \gamma) = h(\theta_{z, \gamma}, z, \gamma)$ ; therefore, $\smoothop(z, \gamma) = \nabla_z h(\theta_{z, \gamma}, z, \gamma) = \theta_{z, \gamma}$.
% \end{proof}

Centralized dual averaging method is explicitly stated in Algorithm~\ref{alg:dual_averaging_standard}.
\begin{algorithm}[t]
  \small
  \caption{Dual averaging algorithm in standard setting.}
  \label{alg:dual_averaging_standard}
  \begin{algorithmic}[1]
    \REQUIRE Step size $(\gamma(t))_{t \geq 0} > 0$ and associated smoothing operator $\smoothop_t$.
    \STATE Initialization $\theta = 0$, $\avtheta = 0$, $z = 0$.
    \FOR{$t = 1, \ldots, T$}
    \STATE Update $z \gets z + g(t)$, where $g(t) \in \nabla \avf(\theta)$
    \STATE Update $\theta \gets \smoothop_t(z)$
    \STATE Update $\avtheta \gets \left( 1 - \frac{1}{t} \right) \avtheta + \frac{1}{t} \theta$
    \ENDFOR
    \RETURN $\avtheta$
  \end{algorithmic}
\end{algorithm}


% The following lemma introduces results similar to Lemma~\ref{lma:inner_prod_bound} for the dual averaging setting.
\begin{lemma}
  \label{lma:bound_inner_dual}
  Let $(u(t))_{t \geq 0}$ be arbitrary sequence of elements in $\bbR^d$ such that $u(0) = 0$ and let $(\gamma(t))_{t \geq 0}$ be a non increasing sequence of elements in $\bbR_+^*$. For $t > 0$, we define $\theta(t)$ as follows:
  \begin{align}
    \theta(t) = \argmin_{\theta' \in \bbR^d} \left\{ \theta'^{\top} \sum_{s = 0}^{t - 1} u(s) + \frac{\| \theta' \|^2}{2 \gamma(t - 1)} + (t-1)\psi(\theta') \right\}.
  \end{align}

  Then, for any $\theta^* \in \bbR^d$ and any $T > 0$, one has:
  \[
    \sum_{t = 1}^T (\theta(t) - \theta^*)^{\top} u(t) \leq \frac{1}{2} \sum_{t = 1}^T \gamma(t - 1) \|u(t)\|^2 + \frac{\|\theta^*\|^2}{2\gamma(T)} + \psi(\theta^*).
  \]
\end{lemma}
\begin{proof}
  For any $\theta \in \bbR^d$ and any $\gamma_1 \geq \gamma_2 > 0$, one has $\frac{1}{2 \gamma_1} \| \theta \|^2 \leq \frac{1}{2 \gamma_2} \| \theta \|^2$, therefore $F(z, \cdot)$ is a non-decreasing function for any $z \in \bbR^d$ and in particular:
  \[
    F\left( \sum_{s = 0}^t u(s), \gamma(t) \right) \geq F\left( \sum_{s = 0}^t u(s), \gamma(t - 1) \right).
  \]
  Lemma~\ref{lma:prox_lipschitz} indicates that $F(\cdot, \gamma)$ is $\gamma$-Lipschitz. Then, for any $y, z \in \bbR^d$, one has $F(z, \gamma) \leq F(y, \gamma) + \smoothop(y, \gamma)^{\top}(z - y) + \frac{\gamma}{2} \|z - y \|^2$; for $z = \sum_{s = 0}^{t - 1} u(s)$ and $y = z + u(t)$, one has:
  \[
    \begin{aligned}
      F\left( \sum_{s = 0}^t u(s), \gamma(t) \right)
      &\geq F\left( \sum_{s = 0}^t u(s), \gamma(t - 1) \right) \\
      &\geq F\left( \sum_{s = 0}^{t - 1} u(s), \gamma(t - 1) \right) + u(t)^{\top} \nabla_z F \left( \sum_{s = 0}^{t - 1} u(s), \gamma(t - 1) \right) - \frac{\gamma(t - 1)}{2} \|u(t) \|^2.
    \end{aligned}
  \]
  Rearranging the terms, we can write with the definition of $\theta(t)$:
  \[
    u(t)^{\top} \theta(t) \leq F\left( \sum_{s = 0}^t u(s), \gamma(t)  \right) - F\left( \sum_{s = 0}^{t- 1} u(s), \gamma(t - 1)  \right) + \frac{\gamma(t - 1)}{2} \|u(t) \|^2.
  \]
  For $T > 0$, the telescopic sum can then be bounded as follows:
  \begin{equation}
    \label{eq:sum_x_bound}
    \sum_{t = 1}^T u(t)^{\top} \theta(t) \leq F\left( \sum_{s = 0}^T u(s), \gamma(T)  \right) - F\left( u(0), \gamma(0)  \right) + \frac{1}{2} \sum_{t = 1}^T \gamma(t - 1) \|u(t) \|^2.
  \end{equation}
  We now provide a bound on the $\theta^*$ part of the sum. By definition of $F$, one has:
  \[
    F\left( \sum_{t = 0}^T u(t), \gamma(T) \right) \leq \left( \sum_{t = 0}^Tu(t) \right)^{\top} \theta^* + \frac{1}{2 \gamma(T)} \| \theta^* \|^2 + \psi(\theta^*),
  \]
  which is equivalent to
  \begin{equation}
    \label{eq:sum_xstar_bound}
    \left( \sum_{t = 0}^T u(t) \right)^{\top} \theta^* \geq F\left( \sum_{t = 0}^T u(t), \gamma(T) \right) - \frac{1}{2\gamma(T)} \|\theta^* \|^2 -\psi(\theta^*).
  \end{equation}
  By combining \eqref{eq:sum_x_bound} and \eqref{eq:sum_xstar_bound}, we finally obtain:
  \[
    \sum_{t = 1}^T (\theta(t) - \theta^*)^{\top} u(t) \leq \frac{1}{2} \sum_{t = 1}^T \gamma(t - 1) \|u(t)\|^2 + \frac{\|\theta^*\|^2}{2\gamma(T)} - F(u(0), \gamma(0)) + u(0)^{\top}\theta^*+ \psi(\theta^*),
  \]
  and the result holds since $u(0) = 0$.
\end{proof}

\begin{theorem}
  Let $(\gamma(t))_{t \geq 0}$ be a non increasing sequence. Let $(z(t))_{t \geq 0}$, $(\theta(t))_{t > 0}$ and $(d(t))_{t > 0}$ be generated according to Algorithm~\ref{alg:dual_averaging_standard}. For $\theta^* \in \argmin_{\theta' \in \bbR^d} \avf(\theta') + \psi(\theta')$ and any $T > 0$, one has:
  \begin{equation}
    \label{eq:dual_standard_bound}
    \avf(\avtheta) + \psi (\avtheta) - \avf(\theta^*) - \psi (\theta^*)  \leq \frac{\| \theta^* \|^2}{2T \gamma(T)} + \frac{L^2}{2T} \sum_{t = 0}^{T - 1} \gamma(t).
  \end{equation}

  Moreover, if there exists $D > 0$ such that for any $y \in \mathcal{Q}$, $\|y\| \leq D$, then for $\gamma(t) = \frac{D}{L \sqrt{2t}}$, one has:
  \[
    \avf( \avtheta) - \avf(\theta^*) \leq \frac{\sqrt{2} D L}{\sqrt{T}} + \frac{L^2}{2T}.
  \]
\end{theorem}



\subsection{Stochastic Dual Averaging}
\label{sec:stoch-subgr-dual}

Similarly to subgradient descent algorithms, one can adapt dual averaging algorithm to a stochastic setting; this setting is deeply studied in \cite{xiao2009dual}. Instead of updating the dual variable $z(t)$ with a subgradient of $\avf$ at $\theta(t)$, one now only requires the \emph{expected} value of the update to be a subgradient, as detailed in Algorithm~\ref{alg:dual_averaging_sto}.
\begin{algorithm}[t]
  \small
  \caption{Dual averaging algorithm in stochastic setting.}
  \label{alg:dual_averaging_sto}
  \begin{algorithmic}[1]
    \REQUIRE Step size $(\gamma(t))_{t \geq 0} > 0$, projection $\smoothop$.
    \STATE Initialization $\theta = 0$, $\avtheta = 0$, $z = 0$.
    \FOR{$t = 1, \ldots, T$}
    \STATE Update $z \gets z + d(t)$, where $\bbE[d(t)|\theta] \in \nabla \avf(\theta)$
    \STATE Update $\theta \gets \smoothop(z, \gamma(t))$
    \STATE Update $\avtheta \gets \left( 1 - \frac{1}{t} \right) \avtheta + \frac{1}{t} \theta$
    \ENDFOR
    \RETURN $ \avtheta $
  \end{algorithmic}
\end{algorithm}
As in the subgradient descent case, convergence results still hold in expectation, as stated in Theorem~\ref{thm:dual_av_sto}.
\begin{theorem}
  \label{thm:dual_av_sto}
  Let $(\gamma(t))_{t \geq 0} \in (\bbR_+^*)^{\bbN}$ be a non increasing sequence. Let $(z(t))_{t \geq 0} \in (\bbR^d)^{\bbN}$, $(\theta(t))_{t > 0} \in (\bbR^d)^{\bbN}$ and $(d(t))_{t > 0} \in (\bbR^d)^{\bbN}$ be generated according to Algorithm~\ref{alg:dual_averaging_sto}. For $\theta^* \in \argmin_{\theta' \in \mathcal{Q}} \avf(\theta')$ and any $T > 0$, one has:
  \begin{equation}
    \label{eq:dual_av_standard_bound}
    \bbE_T\Big[\avf( \avtheta) - \avf(\theta^*)\Big] \leq \frac{\| \theta^* \|^2}{2T \gamma(T)} + \frac{L^2}{2T} \sum_{t = 0}^{T - 1} \gamma(t).
  \end{equation}

  Moreover, if there exists $D > 0$ such that for any $y \in \mathcal{Q}$, $\|y\| \leq D$, then for $\gamma(t) = \frac{D}{L \sqrt{2t}}$, one has:
  \[
    \bbE_T \big[ \avf( \avtheta) - \avf(\theta^*) \big] \leq \frac{\sqrt{2} D L}{\sqrt{T}} + \frac{L^2}{2T}.
  \]
\end{theorem}
\begin{proof}
  As in Theorem~\ref{thm:stochastic_grad_unbiased}, for any $t > 0$, $\theta(t)$ is completely determined by $(d(1), \ldots, d(t - 1))$. Therefore, Lemma~\ref{lma:expected_subgradient} states that inequality~\eqref{eq:gap_general_bound} holds in expectation. Similar reasoning to Lemma~\ref{lma:bound_inner_dual} can be used to finally prove the theorem results.
\end{proof}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../aistats_supp"
%%% End:


==> subfiles/pairwise_function.tex <==
\section{Dual averaging on pairwise functions}
\label{sec:dual-aver-pairw}

Let $(\theta_1, \ldots, \theta_n) \in \Theta^n$ still be $n$ i.i.d.\ realizations of $\theta$ but let us now consider the following problem:
\begin{equation}
\label{eq:ustat_optim}
  \min_{x \in \mathcal{Q}} \frac{1}{n^2} \sum_{1 \leq i, j \leq n} f(x; \theta_i, \theta_j),
\end{equation}
where $f : \mathcal{X} \times \Theta \times \Theta \rightarrow \bbR$ is a convex function. We assume each realization $\theta_i$ is attached to the corresponding node $i$. The goal is for each node to solve problem~\eqref{eq:ustat_optim} using limited memory storage and communication.

\begin{algorithm}[t]
  \small
  \caption{Gossip dual averaging algorithm in synchronous setting.}
  \label{alg:gossip_dual_averaging_sync}
  \begin{algorithmic}[1]
    \REQUIRE Step size $(\gamma(t))_{t \geq 0} > 0$, projection $\nabla_z F$, weights matrix $W$.
    \STATE Each node $i$ initializes $x_i(0) = 0$, $z_i(0) = 0$, $\omega_i(0) = \theta_i$.
    \FOR{$t = 0, \ldots, T - 1$}
    \STATE Draw edge $(i, j)$ uniformly at random
    \STATE Update $Z(t + 1) = W(i, j) Z(t) + D(t)$, where $D(t) =[\nabla_x f(x_1(t); \theta_1, \omega_1(t)), \ldots, \nabla_x f(x_n(t); \theta_n, \omega_n)]$ and $W(i, j) = I_n + \frac{1}{2} (e_i - e_j)(e_i - e_j)^{\top}$
    \FOR{$i = 1, \ldots, n$}
    \STATE Update $x_i(t + 1) = \Pi(z_i(t + 1), \gamma(t))$
    \ENDFOR
    \ENDFOR
    \RETURN $(\overline{x}^T_i)_{1 \leq i \leq n}$
  \end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:gossip_dual_averaging_sync} proposes a way to solve problem~\eqref{eq:ustat_optim}. Each node $i$ stores the primal estimate $x_i$, the dual estimate $z_i$, the parameter $\theta_i$ and an auxiliary parameter $\omega_i$, initialized at $\omega_i = \theta_i$. At each iteration $t$, an edge is drawn at random and the corresponding nodes average their dual estimates and swap their auxiliary parameters. Then, every node $k$ performs an update along a partial gradient estimate $\nabla_x f(x_k(t - 1); \theta_k, \omega_k)$.

Under certain assumptions on $\mathcal{G}$, this method allows to solve problem~\eqref{eq:ustat_optim}, as stated by the following theorem.

\begin{theorem}
  Let $\mathcal{G} = ([n], E)$ be a connected, non bipartite graph. Let $(\gamma(t))_{t \geq 0} \in (\bbR_+^*)^{\bbN}$ be a non increasing sequence. For $i \in [n]$, let $(d_i(t))_{t \geq 0} \in (\bbR^d)^{\bbN}$, $(z_i(t))_{t \geq 0} \in (\bbR^d)^{\bbN}$ and $(x_i(t))_{t > 0} \in (\bbR^d)^{\bbN}$ be generated as stated previously. For $x^* \in \argmin_{x \in \mathcal{Q}} \overline{f}^n(x)$, $i \in [n]$ and $T > 0$, one has:
  \[
    \begin{array}{rcl}
      \bbE_T[\overline{f}^n(\overline{x}^T_i) - \overline{f}^n(x^*)] &\leq & \frac{1}{2 T \gamma(T)} \| x^* \|^2 + \frac{L_f^2}{T}\cdot \frac{2 - \lambda_2(W)}{1 - \lambda_2(W)} \sum_{t = 1}^T \gamma(t - 1) \\
      && + \frac{L_f}{T} \sum_{t = 1}^{T} \bbE_t[\|y(t) - x^*\|] e^{-(1 - \lambda_2(W))t},
    \end{array}
  \]  
  where $\lambda_2(W)$ is the second largest eigenvalue of $W$.
\end{theorem} 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> subfiles/preliminary.tex <==

\section{Preliminary results}
\label{sec:preliminary-results}

\subsection{Preliminary results}
\label{sec:preliminary-results}

Our goal is to solve problem~\eqref{eq:emp_opt_problem} by producing a sequence of elements $(x(t))_{t > 0} \in (\bbR^d)^{\bbN}$ such that $\overline{f}^n(\overline{x}^T)$ is a ``good'' approximation of~\eqref{eq:emp_opt_problem} for $T$ ``large enough''. We state two useful inequalities based on $\overline{f}^n$ convexity. First, for $x^* \in \bbR^d$ and an arbitrary sequence $(x(t))_{t > 0} \in (\bbR^d)^{\bbN}$, one has for $T > 0$:
\begin{equation}
  \label{eq:gap_convexity}
  \overline{f}^n( \overline{x}^T) - \overline{f}^n(x^*)
  = \overline{f}^n \left( \frac{1}{T} \sum_{t = 1}^T x(t) \right) - \overline{f}^n(x^*)
  \leq \frac{1}{T} \sum_{t = 1}^T \big( \overline{f}^n(x(t)) - \overline{f}(x^*) \big).
\end{equation}
This is a direct consequence of convexity definition. Also, for $t > 0$ and $d \in \partial \overline{f}^n(x(t))$, one has:
\begin{equation}
  \label{eq:ineq_subgradient}
  \overline{f}^n(x(t)) - \overline{f}^n(x^*) \leq (x(t) - x^*)^{\top} d.
\end{equation}
Inequality~\eqref{eq:ineq_subgradient} is a consequence of subgradient definition~\eqref{eq:subgradient_prop} and is a key relation for proving algorithms we will introduce. Finally, one can combine both~\eqref{eq:gap_convexity} and \eqref{eq:ineq_subgradient} to write, for $T > 0$:
\begin{equation}
  \label{eq:gap_general_bound}
  \overline{f}^n( \overline{x}^T) - \overline{f}^n(x^*)
  \leq \frac{1}{T} \sum_{t = 1}^T (x(t) - x^*)^{\top} d(t),
\end{equation}
where for any $t \in [T]$, $d(t) \in \partial \overline{f}^n (x(t))$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../aistats_supp"
%%% End:

